Loss-based Bayesian Sequential Prediction of Value at Risk with a Long-Memory and Non-linear Realized Volatility Model

A long memory and non-linear realized volatility model class is proposed for direct Value at Risk (VaR) forecasting. This model, referred to as RNN-HAR, extends the heterogeneous autoregressive (HAR) model, a framework known for efficiently capturing long memory in realized measures, by integrating a Recurrent Neural Network (RNN) to handle non-linear dynamics. Loss-based generalized Bayesian inference with Sequential Monte Carlo is employed for model estimation and sequential prediction in RNN HAR. The empirical analysis is conducted using daily closing prices and realized measures from 2000 to 2022 across 31 market indices. The proposed models one step ahead VaR forecasting performance is compared against a basic HAR model and its extensions. The results demonstrate that the proposed RNN-HAR model consistently outperforms all other models considered in the study.

==> referencelist.tex <==
@article{frazier2024loss,
  title={Loss-based variational {Bayes} prediction},
  author={Frazier, David T and Loaiza-Maya, Ruben and Martin, Gael M and Koo, Bonsoo},
  journal={Journal of Computational and Graphical Statistics},
  number={just-accepted},
  pages={1--31},
  year={2024},
  publisher={Taylor \& Francis}
}
@article{nguyen2022long,
author = {T.-N. Nguyen and M.-N. Tran and D. Gunawan and R. Kohn},
title = {A Statistical Recurrent Stochastic Volatility Model for Stock Markets},
journal = {Journal of Business \& Economic Statistics},
volume = {41},
number = {2},
pages = {414-428},
year  = {2022},
publisher = {Taylor & Francis},
doi = {10.1080/07350015.2022.2028631},
}

@article{del2006sequential,
  title={Sequential {Monte Carlo} samplers},
  author={Del Moral, Pierre and Doucet, Arnaud and Jasra, Ajay},
  journal={Journal of the Royal Statistical Society Series B: Statistical Methodology},
  volume={68},
  number={3},
  pages={411--436},
  year={2006},
  publisher={Oxford University Press}
}
@article{gunawan2022flexible,
  title={Flexible and robust particle tempering for state space models},
  author={Gunawan, David and Kohn, Robert and Tran, Minh Ngoc},
  journal={Econometrics and Statistics},
  year={2022},
  publisher={Elsevier}
}
@article{matsubara2021robust,
  title={Robust generalised Bayesian inference for intractable likelihoods},
  author={Matsubara, Takuo and Knoblauch, Jeremias and Briol, Fran{\c{c}}ois-Xavier and Oates, Chris and others},
  journal={arXiv preprint arXiv:2104.07359},
  year={2021}
}@article{knoblauch2019generalized,
  title={Generalized variational inference: Three arguments for deriving new posteriors},
  author={Knoblauch, Jeremias and Jewson, Jack and Damoulas, Theodoros},
  journal={arXiv preprint arXiv:1904.02063},
  year={2019}
}
@incollection{harvey2007long,
  title={Long memory in stochastic volatility},
  author={Harvey, Andrew C},
  booktitle={Forecasting volatility in the financial markets},
  pages={351--363},
  year={2007},
  publisher={Elsevier}
}

@article{corsi2009simple,
  title={A simple approximate long-memory model of realized volatility},
  author={Corsi, Fulvio},
  journal={Journal of Financial Econometrics},
  volume={7},
  number={2},
  pages={174--196},
  year={2009},
  publisher={Oxford University Press}
}

@article{clements2021practical,
  title={A practical guide to harnessing the har volatility model},
  author={Clements, Adam and Preve, Daniel PA},
  journal={Journal of Banking \& Finance},
  volume={133},
  pages={106285},
  year={2021},
  publisher={Elsevier}
}

@article{arneric2018neural,
  title={Neural network approach in forecasting realized variance using high-frequency data},
  author={Arneri{\'c}, Josip and Poklepovi{\'c}, Tea and Teai, Juin Wen},
  journal={Business Systems Research: International journal of the Society for Advancing Innovation and Research in Economy},
  volume={9},
  number={2},
  pages={18--34},
  year={2018},
  publisher={IRENET, Udruga za promicanje istra{\v{z}}ivanja i inovacija u ekonomiji}
}


@article{corsi2012discrete,
  title={Discrete-time volatility forecasting with persistent leverage effect and the link with continuous-time volatility modeling},
  author={Corsi, Fulvio and Ren{\`o}, Roberto},
  journal={Journal of Business \& Economic Statistics},
  volume={30},
  number={3},
  pages={368--380},
  year={2012},
  publisher={Taylor \& Francis}
}

@article{asai2012asymmetry,
  title={Asymmetry and long memory in volatility modeling},
  author={Asai, Manabu and McAleer, Michael and Medeiros, Marcelo C},
  journal={Journal of Financial Econometrics},
  volume={10},
  number={3},
  pages={495--512},
  year={2012},
  publisher={Oxford University Press}
}


@article{patton2015good,
  title={Good volatility, bad volatility: Signed jumps and the persistence of volatility},
  author={Patton, Andrew J and Sheppard, Kevin},
  journal={Review of Economics and Statistics},
  volume={97},
  number={3},
  pages={683--697},
  year={2015},
  publisher={The MIT Press}
}


@article{bollerslev2016exploiting,
  title={Exploiting the errors: A simple approach for improved volatility forecasting},
  author={Bollerslev, Tim and Patton, Andrew J and Quaedvlieg, Rogier},
  journal={Journal of Econometrics},
  volume={192},
  number={1},
  pages={1--18},
  year={2016},
  publisher={Elsevier}
}


@article{huang2016modeling,
  title={Modeling long memory volatility using realized measures of volatility: A realized {HAR GARCH} model},
  author={Huang, Zhuo and Liu, Hao and Wang, Tianyi},
  journal={Economic Modelling},
  volume={52},
  pages={812--821},
  year={2016},
  publisher={Elsevier}
}

@article{corsi2008volatility,
  title={The volatility of realized volatility},
  author={Corsi, Fulvio and Mittnik, Stefan and Pigorsch, Christian and Pigorsch, Uta},
  journal={Econometric Reviews},
  volume={27},
  number={1-3},
  pages={46--78},
  year={2008},
  publisher={Taylor \& Francis}
}

@article{nguyen2022recurrent,
  title={Recurrent conditional heteroskedasticity},
  author={Nguyen, Trong-Nghia and Tran, Minh-Ngoc and Kohn, Robert},
  journal={Journal of Applied Econometrics},
  volume={37},
  number={5},
  pages={1031--1054},
  year={2022},
  publisher={Wiley Online Library}
}

@article{fissler2016higher,
  title={Higher order elicitability and {Osband’s} principle},
  author={Fissler, Tobias and Ziegel, Johanna F},
  journal   = {The Annals of Statistics},
  year      = {2016},
  number    = {4},
  pages     = {1680--1707},
  volume    = {44},
}


@article{bissiri2016general,
  title={A general framework for updating belief distributions},
  author={Bissiri, Pier Giovanni and Holmes, Chris C and Walker, Stephen G},
  journal={Journal of the Royal Statistical Society Series B: Statistical Methodology},
  volume={78},
  number={5},
  pages={1103--1130},
  year={2016},
  publisher={Oxford University Press}
}


@article{taylor2019forecasting,
  title={Forecasting value at risk and expected shortfall using a semiparametric approach based on the asymmetric {Laplace} distribution},
  author={Taylor, James W},
  journal={Journal of Business \& Economic Statistics},
  volume={37},
  number={1},
  pages={121--133},
  year={2019},
  publisher={Taylor \& Francis}
}


@article{heber2009omi,
  title={Oxford-Man Institute's realized library, version 0.3},
  author={Heber, Gerd and Lunde, Asger and Shephard, Neil and Sheppard, Kevin},
  journal={Oxford-Man Institute, University of Oxford},
  year={2009}
}

@article{engle2004caviar,
  title={CAViaR: Conditional autoregressive value at risk by regression quantiles},
  author={Engle, Robert F and Manganelli, Simone},
  journal={Journal of business \& economic statistics},
  volume={22},
  number={4},
  pages={367--381},
  year={2004},
  publisher={Taylor \& Francis}
}
@article{Kim:2018,
	title = "Forecasting the volatility of stock price index: A hybrid model integrating {LSTM} with multiple {GARCH-type} models",
	journal = "Expert Systems with Applications",
	volume = "103",
	pages = "25 - 37",
	year = "2018",
	issn = "0957-4174",
	doi = "https://doi.org/10.1016/j.eswa.2018.03.002",
	url = "http://www.sciencedirect.com/science/article/pii/S0957417418301416",
	author = "Ha Young Kim and Chang Hyun Won",
	keywords = "LSTM, GARCH, Deep learning, Volatility prediction, Hybrid model",
}
@article{gerlach2016bayesianB,
  title={Bayesian assessment of dynamic quantile forecasts},
  author={Gerlach, Richard and Chen, Cathy WS and Lin, Edward MH},
  journal={Journal of Forecasting},
  volume={35},
  number={8},
  pages={751--764},
  year={2016},
  publisher={Wiley Online Library}
}

@article{de2019minimum,
  title={Minimum capital requirements for market risk},
  author={BCBS},
  journal={Suiza: BCBS},
  year={2019}
}


@article{hansen2005forecast,
  title={A forecast comparison of volatility models: does anything beat a {GARCH} (1,1)?},
  author={Hansen, Peter R and Lunde, Asger},
  journal={Journal of applied econometrics},
  volume={20},
  number={7},
  pages={873--889},
  year={2005},
  publisher={Wiley Online Library}
}

@article{gerlach2011bayesian,
  title={Bayesian time-varying quantile forecasting for value-at-risk in financial markets},
  author={Gerlach, Richard H and Chen, Cathy WS and Chan, Nancy YC},
  journal={Journal of business \& economic statistics},
  volume={29},
  number={4},
  pages={481--492},
  year={2011},
  publisher={Taylor \& Francis}
}

@article{bucci2020realized,
  title={Realized volatility forecasting with neural networks},
  author={Bucci, Andrea},
  journal={Journal of Financial Econometrics},
  volume={18},
  number={3},
  pages={502--531},
  year={2020},
  publisher={Oxford University Press}
}

@article{almosova2023nonlinear,
  title={Nonlinear inflation forecasting with recurrent neural networks},
  author={Almosova, Anna and Andresen, Niek},
  journal={Journal of Forecasting},
  volume={42},
  number={2},
  pages={240--259},
  year={2023},
  publisher={Wiley Online Library}
}

@article{lipton2015criticalreview,
  title={A Critical Review of Recurrent Neural Networks for Sequence Learning},
  author={Lipton,Zachary C. and Berkowitz,John and Elkan,Charles},
  journal={ProQuest One Academic},
  year={2015},
  publisher={ArXiv.Org}
}

@article{chronopoulos2023forecasting,
  title={Forecasting value-at-risk using deep neural network quantile regression},
  author={Chronopoulos, Ilias and Raftapostolos, Aristeidis and Kapetanios, George},
  journal={Journal of financial econometrics},
  pages={nbad014},
  year={2023},
  publisher={Oxford University Press}
}


@article{qiu2024var,
  title={VaR and ES forecasting via recurrent neural network-based stateful models},
  author={Qiu, Zhiguo and Lazar, Emese and Nakata, Keiichi},
  journal={International Review of Financial Analysis},
  volume={92},
  pages={103102},
  year={2024},
  publisher={Elsevier}
}


@article{baillie1996fractionally,
  title={Fractionally integrated generalized autoregressive conditional heteroskedasticity},
  author={Baillie, Richard T and Bollerslev, Tim and Mikkelsen, Hans Ole},
  journal={Journal of econometrics},
  volume={74},
  number={1},
  pages={3--30},
  year={1996},
  publisher={Elsevier}
}
%  1
@article{bollerslev1986generalized,
  title={Generalized autoregressive conditional heteroskedasticity},
  author={Bollerslev, Tim},
  journal={Journal of econometrics},
  volume={31},
  number={3},
  pages={307--327},
  year={1986},
  publisher={Elsevier}
}
% 1
@book{taylor2008modeling,
    author = {Taylor, S},
    title = {Modelling financial time series},
    publisher = {World Scientific},
    year = {2008},}
}{taylor2008modeling,
  title={Modeling financial time series john wiley \& sons},
  author={Taylor, S},
  journal={Great Britain},
  volume={10},
  pages={20--34},
  year={2008}
}
% 1
@article{andersen2003modeling,
  title={Modeling and forecasting realized volatility},
  author={Andersen, Torben G and Bollerslev, Tim and Diebold, Francis X and Labys, Paul},
  journal={Econometrica},
  volume={71},
  number={2},
  pages={579--625},
  year={2003},
  publisher={Wiley Online Library}
}

@article{cont2001empirical,
  title={Empirical properties of asset returns: stylized facts and statistical issues},
  author={Cont, Rama},
  journal={Quantitative finance},
  volume={1},
  number={2},
  pages={223},
  year={2001},
  publisher={IOP Publishing}
}

@book{tsay2010analysis,
  title={Analysis of financial time series},
  author={Tsay, Ruey S},
  year={2010},
  publisher={John Wiley \& sons}
}

@book{frey2010quantitative,
  title={Quantitative risk management},
  author={Frey, Rudiger and Embrechts, Paul},
  year={2010},
  publisher={Princeton University Press}
}

@book{christoffersen2011elements,
  title={Elements of financial risk management},
  author={Christoffersen, Peter},
  year={2011},
  publisher={Academic press}
}


@article{jewson2022general,
  title={General Bayesian loss function selection and the use of improper models},
  author={Jewson, Jack and Rossell, David},
  journal={Journal of the Royal Statistical Society Series B: Statistical Methodology},
  volume={84},
  number={5},
  pages={1640--1665},
  year={2022},
  publisher={Oxford University Press}
}
%Lipton, Zachary C, et al. “A Critical Review of Recurrent Neural Networks for Sequence %Learning.” ArXiv.Org, Ithaca, 2015. ProQuest One Academic, Accessed 2 June 2024. 



%%%%%%%%%%update 21%%%%%%%%%%%%%%%%%%%
%article{ChristensenKim2022AMLA,
author = {Christensen, Kim and Siggaard, Mathias and Veliyev, Bezirgen},
issn = {1479-8409},
journal = {Journal of financial econometrics},
language = {eng},
title = {A Machine Learning Approach to Volatility Forecasting},
year = {2022},
}



%article{masini2023machine,
  title={Machine learning advances for time series forecasting},
  author={Masini, Ricardo P and Medeiros, Marcelo C and Mendes, Eduardo F},
  journal={Journal of economic surveys},
  volume={37},
  number={1},
  pages={76--111},
  year={2023},
  publisher={Wiley Online Library}
}



%% article{vortelinos2017forecasting,
%  title={Forecasting realized volatility: HAR against Principal Components Combining, neural networks and GARCH},
  author={Vortelinos, Dimitrios I},
  journal={Research in international business and finance},
  volume={39},
  pages={824--839},
  year={2017},
  publisher={Elsevier}
%}


% article{chen2023tail,
 % title={Tail risk forecasting of realized volatility CAViaR models},
  author={Chen, Cathy WS and Hsu, Hsiao-Yun and Watanabe, Toshiaki},
  journal={Finance Research Letters},
  volume={51},
  pages={103326},
  year={2023},
  publisher={Elsevier}
%}


% article{tran2021variational,
  title={Variational Bayes on manifolds},
  author={Tran, Minh-Ngoc and Nguyen, Dang H and Nguyen, Duy},
  journal={Statistics and Computing},
  volume={31},
  pages={1--17},
  year={2021},
  publisher={Springer}
}

%article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

%article{li2020bayesian,
  title={A bayesian long short-term memory model for value at risk and expected shortfall joint forecasting},
  author={Li, Zhengkun and Tran, Minh-Ngoc and Wang, Chao and Gerlach, Richard and Gao, Junbin},
  journal={arXiv preprint arXiv:2001.08374},
  year={2020}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old paper references



%article{chen2006comparison,
  title={Comparison of nonnested asymmetric heteroskedastic models},
  author={Chen, Cathy WS and Gerlach, Richard and So, Mike KP},
  journal={Computational Statistics \& Data Analysis},
  volume={51},
  number={4},
  pages={2164--2178},
  year={2006},
  publisher={Elsevier}
}

%article{bradley1996ramanujan,
  title={Ramanujan's formula for the logarithmic derivative of the gamma function},
  author={Bradley, David},
  booktitle={Mathematical Proceedings of the Cambridge Philosophical Society},
  volume={120},
  number={3},
  pages={391--401},
  year={1996},
  organization={Cambridge University Press}
}

%inproceedings{ari2018bayesian,
  title={Bayesian Estimation of GARCH (1, 1) Model Using Tierney-Kadane’s Approximation},
  author={Ar{\i}, Yakup},
  booktitle={International Conference on Applied Economics},
  pages={355--364},
  year={2018},
  organization={Springer}
}

%article{sebah2002introduction,
  title={Introduction to the gamma function},
  author={Sebah, Pascal and Gourdon, Xavier},
  journal={American Journal of Scientific Research},
  pages={2--18},
  year={2002}
}

%article{gefang2022forecasting,
  title={Forecasting using variational Bayesian inference in large vector autoregressions with hierarchical shrinkage},
  author={Gefang, Deborah and Koop, Gary and Poon, Aubrey},
  journal={International Journal of Forecasting},
  year={2022},
  publisher={Elsevier}
}


%online{MathMLE,
  author = {The MathWorks, Inc.},
  title = {Maximum Likelihood Estimation for Conditional Variance Models},
  year = 1999,
  url = {https://au.mathworks.com/help/econ/maximum-likelihood-estimation-for-conditional-variance-models.html},
  urldate = {2022-09-19}
}

%  % article{lipton2015critical,
%  title={A critical review of recurrent neural networks for sequence learning},
  author={Lipton, Zachary C and Berkowitz, John and Elkan, Charles},
  journal={arXiv preprint arXiv:1506.00019},
  year={2015}
%}







